A Pendulum-Driven Legless Rolling Jumping Robot

In this paper, we present a novel rolling, jumping robot. The robot consists of a driven pendulum mounted to a wheel in a compact, lightweight, 3D printed design. We show that by driving the pendulum to shift the robot's weight distribution, the robot is able to obtain significant rolling speed, achieve jumps of up to 2.5 body lengths vertically, and clear horizontal distances of over 6 body lengths. The robot's dynamic model is derived and simulation results indicate that it is consistent with the rolling motion and jumping observed on the robot. The ability to both roll and jump effectively using a minimalistic design makes this robot unique and could inspire the use of similar mechanisms on robots intended for applications in which agile locomotion on unstructured terrain is necessary, such as disaster response or planetary exploration.

==> horjump_fig.tex <==
        \begin{tikzpicture}%
            \node[anchor=south west,inner sep=0] (f) at (0,0) {\includegraphics[width = 0.19\linewidth]{oh207_crop.jpg}};
            \draw [very thin] (f.north east) rectangle (f.south west);
            \draw [thin, red] (0.49,0.9) -- ++(0,-0.25); 
        \end{tikzpicture}
        \begin{tikzpicture}%
            \node[anchor=south west,inner sep=0] (f) at (0,0) {\includegraphics[width = 0.19\linewidth]{oh245_crop.jpg}};
            \draw [very thin] (f.north east) rectangle (f.south west);
            % \draw [thin, -{Latex[length=2pt]}, red] (0.49,0.9) -- ++(0,-0.25); 
            % \draw [thin, -{Latex[length=2pt]}, blue] (1.07,0.9) -- ++(0,-0.25); 
        \end{tikzpicture}
        \begin{tikzpicture}%
            \node[anchor=south west,inner sep=0] (f) at (0,0) {\includegraphics[width = 0.19\linewidth]{oh264_crop.jpg}};
            \draw [very thin] (f.north east) rectangle (f.south west);
            \draw [thin, red] (0.49,0.9) -- ++(0,-0.25); 
            \draw [thin, red] (1.5,0.9) -- ++(0,-0.25); 
            \draw [thin, red, latex-latex] (0.49,0.9-0.125) -- (1.5,0.9-0.125);
        \end{tikzpicture}
        \begin{tikzpicture}%
            \node[anchor=south west,inner sep=0] (f) at (0,0) {\includegraphics[width = 0.19\linewidth]{oh322_crop.jpg}};
            \draw [very thin] (f.north east) rectangle (f.south west);
        \end{tikzpicture}
        \begin{tikzpicture}%
            \node[anchor=south west,inner sep=0] (f) at (0,0) {\includegraphics[width = 0.19\linewidth]{oh359_crop.jpg}};
            \draw [very thin] (f.north east) rectangle (f.south west);
            % \draw [thin, red] (0.49,0.9) -- ++(0,-0.25); 
            \draw [thin, red] (1.5,0.9) -- ++(0,-0.35); 
            \draw [thin, red] (3.25,0.9) -- ++(0,-0.35); 
            \draw [thin, red, latex-latex] (1.5,0.9-0.125) -- (3.25,0.9-0.125);
        \end{tikzpicture}
            % \includegraphics[width = 0.19\linewidth]{oh207_crop.jpg}
            % \includegraphics[width = 0.19\linewidth]{oh245_crop.jpg}
            % \includegraphics[width = 0.19\linewidth]{oh264_crop.jpg}
            % \includegraphics[width = 0.19\linewidth]{oh322_crop.jpg}
            % \includegraphics[width = 0.19\linewidth]{oh359_crop.jpg}
            \\[1ex]
            \begin{tikzpicture}%
            \node[anchor=south west,inner sep=0] (f) at (0,0) {\includegraphics[width = 0.19\linewidth]{0207_crop.jpg}};
                \draw [very thin] (f.north east) rectangle (f.south west);
                \node (C) at ($(f.south east)!0.5!(f.south west)+(0,-0.3)$) {(a)};
                % \node at (C)++(0,-0.2) {a};
                
            \end{tikzpicture}
            \begin{tikzpicture}%
                \node[anchor=south west,inner sep=0] (f) at (0,0) {\includegraphics[width = 0.19\linewidth]{0245_crop.jpg}};
                \draw [very thin] (f.north east) rectangle (f.south west);
                \node (C) at ($(f.south east)!0.5!(f.south west)+(0,-0.3)$) {(b)};
                \end{tikzpicture}
            \begin{tikzpicture}%
                \node[anchor=south west,inner sep=0] (f) at (0,0) {\includegraphics[width = 0.19\linewidth]{0264_crop.jpg}};
                \draw [very thin] (f.north east) rectangle (f.south west);
                \node (C) at ($(f.south east)!0.5!(f.south west)+(0,-0.3)$) {(c)};
            \end{tikzpicture}
            \begin{tikzpicture}%
                \node[anchor=south west,inner sep=0] (f) at (0,0) {\includegraphics[width = 0.19\linewidth]{0322_crop.jpg}};
                \draw [very thin] (f.north east) rectangle (f.south west);
                \node (C) at ($(f.south east)!0.5!(f.south west)+(0,-0.3)$) {(d)};
            \end{tikzpicture}
            \begin{tikzpicture}%
                \node[anchor=south west,inner sep=0] (f) at (0,0) {\includegraphics[width = 0.19\linewidth]{0359_crop.jpg}};
                \draw [very thin] (f.north east) rectangle (f.south west);
                \node (C) at ($(f.south east)!0.5!(f.south west)+(0,-0.3)$) {(e)};
            \end{tikzpicture}
		    % \includegraphics[width = 0.19\linewidth]{0207_crop.jpg}
      %       \includegraphics[width = 0.19\linewidth]{0245_crop.jpg}
      %       \includegraphics[width = 0.19\linewidth]{0264_crop.jpg}
      %       \includegraphics[width = 0.19\linewidth]{0322_crop.jpg}
      %       \includegraphics[width = 0.19\linewidth]{0359_crop.jpg}
